Enjoying the Product but Not Joining the Builders: Investigating Why Students Don't Contribute to OSS

Open-source software (OSS) participation provides students with authentic exposure to collaborative, real-world software development, yet active contributions remain limited. This short paper presents an exploratory study of computing students' perceptions, knowledge, and experiences with OSS at the University of Hawai'i at Manoa. We administered a survey and analyzed 122 responses using both quantitative and qualitative methods. Students reported moderate OSS familiarity and frequent OSS use in coursework and personal projects, yet only 12.3% actively contributed and engagement with OSS communities was limited. Key barriers included skill gaps (72.89% of non-contributors), time constraints (59.81%), and codebase complexity (66.67% of contributors), often alongside imposter syndrome (36.45%). Students indicated that more time, mentorship, beginner-friendly issues, better onboarding/documentation, and curricular incentives (e.g., course credit) would most increase participation, while most reported their courses do not require or incentivize OSS contributions (58.20%). Grounded in a single institutional context, this study provides a nuanced understanding of how curriculum structure, faculty encouragement, and competing academic demands shape OSS participation. These insights inform the design of targeted curricular and institutional interventions aimed at supporting student onboarding and participation in OSS communities.

==> tables/demographics/Academic_Standing.tex <==
\begin{table}[H]
\caption{Distribution of Academic Standing }
\label{tab:academic-standing}
\begin{tabular}{lll}
\hline
Class Standing                  & Count & Percentage \\ \hline
Undergraduate - 3rd year           & 45    & 36.89\%    \\ \hline
Undergraduate - 4th year           & 24    & 19.67\%    \\ \hline
Undergraduate - 2nd year           & 19    & 15.57\%    \\ \hline
Graduate student (Master's)        & 17    & 13.93\%    \\ \hline
Undergraduate - 5th year or beyond & 11    & 9.02\%     \\ \hline
Graduate student (Ph.D.)           & 5     & 4.10\%     \\ \hline
Undergraduate - 1st year           & 1     & 0.82\%     \\ \hline
\end{tabular}
\end{table}
